Object-Centric Vision Token Pruning for Vision Language Models

In Vision Language Models (VLMs), vision tokens are quantity-heavy yet information-dispersed compared with language tokens, thus consume too much unnecessary computation. Pruning redundant vision tokens for high VLM inference efficiency has been continuously studied but all existing methods resort to indirect and non-guaranteed ways. We propose OC-VTP, a direct and guaranteed approach to select the most representative vision tokens for high-efficiency yet accuracy-preserving VLM inference. Our OC-VTP requires merely light-weight pre-training of a small object-centric vision token pruner, which can then be inserted into existing VLMs, without fine-tuning of any models on any datasets. It is gauranteed that the most representative vision tokens are kept by minimizing the error in reconstructing the original unpruned tokens from the selected ones. Across any vision pruning ratios, i.e., inference efficiency, our OC-VTP consistently helps mainstream VLMs to preserve the highest inference accuracy. Our pruning also demonstrates interesting interpretability. Our codes are available at https://github.com/GarryLarry010131/OC-VTP.

==> equations/InverseAreaRatio.tex <==
\begin{equation}
  \text{area}_s=\sum_t{\alpha_{s,t}}
  \label{eq:Areas}
\end{equation}

\begin{equation}
    r_s=\text{area}_s/T
    \label{eq:AreasRatio}
\end{equation}

\begin{equation}
    w_s=\big(\max\{r_s,\varepsilon\}\big)^{-p}
    \label{eq:InverseAreasRatio}
\end{equation}


==> equations/MSELoss.tex <==
\begin{equation}
  \mathcal{L}_{\mathrm{rec}}=\|X-\hat X\|^2
  \label{eq:MSELoss}
\end{equation}

==> equations/WeightedAlpha.tex <==
\begin{equation}
    \alpha^{\text{final}}_t=\sum_{s=1}^{S} w_s\,\alpha_{s,t}\
    \label{eq:AlphaFinal}
\end{equation}


==> images_tex/method_ocl_pipeline.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.96\linewidth]{images/Method_OCL_Pipeline.pdf}
\caption{
\textbf{OC-Pruner training pipeline.}
Given input features $X\in\mathbb{R}^{T\times d}$, $S$ slots are sampled from a learned Gaussian distribution. Slot Attention inputs slots and tokens, then yields an attention map $A\in\mathbb{R}^{S\times T}$ and slot embeddings $Z\in\mathbb{R}^{S\times d}$. A lightweight Transformer decoder reconstructs token features $\hat X=D(Z)$. The model is trained using the reconstruction loss.
}
\label{fig:Ocl_Pipeline}
\end{figure}


==> rebuttal_images/dead_slots.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.75\linewidth]{rebuttal_images/dead_slots.pdf}
  \caption{Distribution of \textbf{effective slot} usage during inference.}
  \label{fig:dead_slots}
\end{figure}


==> rebuttal_tables/resize.tex <==
% \begin{table}
%   \caption{Results.   Ours is better.}
%   \label{tab:llava1.5Acc}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table}[]
    \centering
    \resizebox{0.4\textwidth}{!}{
    \begin{tabular}{l|cccccc|c}
        \toprule
        Method & MMB & POPE & SQA & VizWiz & InfoVQA & ChartQA & Avg \\
        \midrule
        \multicolumn{8}{c}{Vanilla, \textbf{100\%} Tokens} \\
        \multirow{2}{*}{Qwen2.5-VL-7B} & 77.3 & 87.0 & 80.4 & 68.3 & 80.3 & 83.8 & \multirow{2}{*}{100\%} \\
        & {\scriptsize 100\%} & {\scriptsize 100\%} & {\scriptsize 100\%} & {\scriptsize 100\%} & {\scriptsize 100\%} & {\scriptsize 100\%}\\
        \midrule

        \multicolumn{8}{c}{Retain \textbf{11.1\%} Tokens} \\

        \multirow{2}{*}{Resize} & \textbf{72.1} & 81.3 & \textbf{78.2} & \textbf{64.9} & 59.5 & 33.5 & \multirow{2}{*}{82.2\%} \\
        & {\scriptsize \textbf{93.3\%}} & {\scriptsize 93.4\%} & {\scriptsize \textbf{97.3\%}} & {\scriptsize \textbf{95.0\%}} & {\scriptsize 74.1\%} & {\scriptsize 40.0\%} \\ 

        \midrule
        \multirow{2}{*}{\textbf{OC-VTP$^{\text{Ours}}$}} & 70.9 & \textbf{81.8} & 78.0 & 64.2 & \textbf{65.6} & \textbf{53.7} & \multirow{2}{*}{\textbf{87.1\%}} \\
        & {\scriptsize 91.7\%} & {\scriptsize \textbf{94.0\%}} & {\scriptsize 97.0\%} & {\scriptsize 94.0\%} & {\scriptsize \textbf{81.7\%}} & {\scriptsize \textbf{64.1\%}} \\  
        \bottomrule
    \end{tabular}
    }
    \caption{Comparison between the \textbf{\emph{Resize operation} baseline} and OC-VTP, with additional evaluations on \textbf{text-rich benchmarks}.}
    \label{tab:resize}
\end{table}


==> rebuttal_tables/video_ocr.tex <==
\setlength{\aboverulesep}{0em}  % Space above mid and bottom rules
\setlength{\belowrulesep}{0em}

\begin{table}[]
    \small
    \centering
    \resizebox{0.24\textwidth}{!}{
\begin{tabular}{l|cc|c}
\toprule
Method & MSVD & MSRVTT & Avg \\
        \midrule
        \multicolumn{4}{c}{Vanilla, 2048 Tokens (\textbf{100\%})} \\
        \multirow{2}{*}{Video-LLaVA} & 70.2 & 57.4 & \multirow{2}{*}{100\%} \\
        & {\scriptsize 100\%} & {\scriptsize 100\%}\\
        \midrule

        \multicolumn{4}{c}{Retain 136 Tokens (\textbf{6.6\%})} \\

        \multirow{2}{*}{VisionZip} & 63.5 & 52.1 & \multirow{2}{*}{90.7\%} \\
        & {\scriptsize 90.5\%} & {\scriptsize 90.8\%} \\ 
        \midrule

        \multirow{2}{*}{OC-VTP} & \textbf{63.6} & \textbf{52.9} & \multirow{2}{*}{\textbf{91.4\%}} \\
        & {\scriptsize \textbf{90.6\%}} & {\scriptsize \textbf{92.2\%}} \\ 
        \bottomrule
\end{tabular}
}
\caption{Comparison on \textbf{video-understanding benchmarks}.}
\label{tab:video}
\end{table}
